A suite of allotaxonometric tools for the comparison of complex systems using rank-turbulence divergence

Describing and comparing complex systems requires principled, theoretically grounded tools. Built around the phenomenon of type turbulence, allotaxonographs provide map-and-list visual comparisons of pairs of heavy-tailed distributions. Allotaxonographs are designed to accommodate a wide range of instruments including rank- and probability-turbulence divergences, Jenson-Shannon divergence, and generalized entropy divergences. Here, we describe a suite of programmatic tools for rendering allotaxonographs for rank-turbulence divergence in Matlab, Javascript, and Python, all of which have different use cases.

==> allotaxonometer-for-everyone.changelog.tex <==
%% for arXivs of the various stripes

\todo{Notes on what has changed}
- 22Sept2025: base URL changed for UVM's complex stories. Updated here.
